Estimating Discretization Error with Preset Orders of Accuracy and Fractional Refinement Ratios

Verification of solutions is crucial for establishing the reliability of simulations. A central challenge is to find an accurate and reliable estimate of the discretization error. Current approaches to this estimation rely on the observed order of accuracy; however, studies have shown that it may alter irregularly or become undefined. Therefore, we propose a grid refinement method which adopts constant orders given by the user, called the Preset Orders Expansion Method (POEM). The user is guaranteed to obtain the optimal set of orders through iterations and hence an accurate estimate of the discretization error. This method evaluates the reliability of the estimation by assessing the convergence of the expansion terms, which is fundamental for all grid refinement methods. We demonstrate these capabilities using advection and diffusion problems along different refinement paths. POEM requires a lower computational cost when the refinement ratio is higher. However, the estimated error suffers from higher uncertainty due to the reduced number of shared grid points. We circumvent this by using fractional refinement ratios and the Method of Interpolating Differences between Approximate Solutions (MIDAS). As a result, we can obtain a global estimate of the discretization error of lower uncertainty at a reduced computational cost.

==> sections/old_ReviewGRE.tex <==
\section{Review of the Generalized Richardson Extrapolation} \label{sec:review_GRE}
When $\phi_{e}$ is smooth over the domain of the mathematical model, we can expand $\phi$ about $\phi_{e}$ in a power series at every grid point to obtain
\begin{equation} \label{eq:model_orig}
    \phi = \phi_{e} + \sum_{m=1}^{\infty} C_{q_m} h^{q_m},
\end{equation}
where the coefficients $\{C_{q}\}$ are functions of space and time but not the grid spacing $h$, and the orders $\{q_m: q_1 < q_2 < \dots \}$ are integers determined by the choice of the numerical scheme. In particular, $q_1$ is the formal (theoretical) order of accuracy of the numerical scheme. Here $C_{q} h^{q}$ represents the sum of all the coefficient terms of order $q$. Its specific form will be clarified in Section \ref{subsec:1+1_dim}.

In the generalized Richardson extrapolation \citep{Roache1994Perspective:Studies,Roy2010}, the series of coefficient terms is modeled by a single coefficient term:
\begin{equation} \label{eq:coef_term_GRE}
    C_{\Tilde{q}} h^{\Tilde{q}} = \sum_{m=1}^{\infty} C_{q_m} h^{q_m},
\end{equation}
where $C_{\Tilde{q}}$ and ${\Tilde{q}}$ are unknowns to be determined. Moreover, as this work is concerned with solution verification, ${\phi}_{e}$ is replaced by $\Tilde{\phi}_{e}$. Therefore,
\begin{equation}
    \phi = \Tilde{\phi}_{e} + C_{\Tilde{q}} h^{\Tilde{q}}.
\end{equation}
The exponent $\Tilde{q}$ is known as the observed order of accuracy. Unlike $\{q_m\}$, it is generally not an integer. In fact, it is because of this non-integer nature that $C_{\Tilde{q}} h^{\Tilde{q}}$ can map to any real number and therefore model the series of coefficient terms accurately.

To solve for $\{\Tilde{\phi}_{e}, C_{\Tilde{q}}, {\Tilde{q}}\}$ uniquely, solutions on three systematically-refined grids are required \citep{Roy2010}. Consider such a set of grids, where the refinement ratio $r \in [0.5,1)$ is uniform over the domain and constant across refinement levels. Let $\phi_1, \phi_2, \phi_3$ be the solution on the coarse, medium, and fine grid respectively. Then, we have
\begin{align}
    \phi_1 &= \Tilde{\phi}_{e} + C_{\Tilde{q}} h^{\Tilde{q}}, \\
    \phi_2 &= \Tilde{\phi}_{e} + C_{\Tilde{q}} (r h)^{\Tilde{q}}, \\
    \phi_3 &= \Tilde{\phi}_{e} + C_{\Tilde{q}} (r^2 h)^{\Tilde{q}}.
\end{align}
This system of equations has the solution
\begin{align}
    \Tilde{\phi}_{e} &= \phi_1 - C_{\Tilde{q}} h^{\Tilde{q}}, \\
    \Tilde{q} &= \ln \Big( \frac{\phi_3 - \phi_2}{\phi_2 - \phi_1} \Big) / \ln r, \label{eq:q_tilde} \\
    C_{\Tilde{q}} h^{\Tilde{q}} &= \frac{\phi_2 - \phi_1}{r^{\Tilde{q}} - 1}.
\end{align}
As a result, the estimated DE is given by
\begin{equation}
    \Tilde{\varepsilon} = \phi_1 - \Tilde{\phi_{e}} = \frac{\phi_2 - \phi_1}{r^{\Tilde{q}} - 1}.
\end{equation}

The reliability of DE estimation in grid refinement methods is associated with the concept of asymptotic range \citep{Roy2010}. The asymptotic range is defined as the sequence of grids over which the DE reduces at the formal order of accuracy. This is achieved when the grid spacing, $h$, is sufficiently small that the leading order term ($m=1$) dominates the series of coefficient terms in Equation \ref{eq:model_orig}. In this case, Equation \ref{eq:coef_term_GRE} reduces to linear maps, i.e. $C_{\Tilde{q}} \mapsto C_{q_1}$ and $\Tilde{q} \mapsto q_1$. Because of this, the DE estimation is considered reliable.

However, using the observed order of accuracy for DE estimation has two potential problems. First, since the observed order, $\Tilde{q}$, is the exponent of the coefficient term, $C_{\Tilde{q}} h^{\Tilde{q}}$, the estimated DE behaves non-linearly as the observed order changes. A small variation of the value can lead to irregular alteration of the estimated DE \citep{Roy2003,Eca2009,Hodis2012GridAneurysms}. Second, when the sign of $\phi_3 - \phi_2$ and $\phi_2 - \phi_1$ are different, the value of $\Tilde{q}$ is undefined according to Equation \ref{eq:q_tilde}. This can happen in the vicinity of an abrupt change, for example, a shock wave \citep{Roy2003}. A remedy of these problems is to limit $\Tilde{q}$ in a range \citep{OberkampfRoy2010}; however, the estimated DE may then contain unpredictable errors.

The observed order of accuracy is also the basis of many approaches to evaluating the uncertainty of the estimated DE \citep{Orozco2010VerificationSolutions,Phillips2014RichardsonDynamics}. Due to the aforementioned problems, the uncertainty estimate may also contain unpredictable errors. From a more fundamental viewpoint, the problem originates from the failure of asymptotic convergence of the approximate solutions \citep{Roy2010}. The reliability of the DE estimation is highly questionable in this case. Therefore, we focus on assessing the reliability rather than evaluating the uncertainty of DE estimates.

%------------------------------------------------------------------------------
